Novi jezi\v{c}ki modeli za srpski jezik

The paper will briefly present the development history of transformer-based language models for the Serbian language. Several new models for text generation and vectorization, trained on the resources of the Society for Language Resources and Technologies, will also be presented. Ten selected vectorization models for Serbian, including two new ones, will be compared on four natural language processing tasks. Paper will analyze which models are the best for each selected task, how does their size and the size of their training sets affect the performance on those tasks, and what is the optimal setting to train the best language models for the Serbian language.

==> chapters/1.tex <==
\section{Увод}
\label{sec:1}


Почетком двадесет и првог века, дошло је најпре до наглог пораста количине доступних текстуалних података, а потом и до наглог раста рачунарске моћи, што је покренуло талас истраживања заснованих на идеји дубоког учења (\textit{deep learning})~\autocite{lecun2015deep}. У случају обраде природних језика, истраживања кулминирају појавом архитектуре трансформера~\citep{vaswani2017attention}, која се базира на употреби енкодера, чија је главна намена анализа тескта, и декодера, чија је главна намена синтеза тескта. Ипак, први опште популаран модел базиран на овој архитектури био је \textit{BERT}\footnote{\textit{Bidirectional Encoder Representations from Transformers} -- двосмерно кодирање репрезентације из трансформера}~\citep{devlin2018bert}, заснован искључиво на трансформерском енкодеру. Овај модел је направио велики помак у обради природног језика, пре свега на задацима који се заснивају на векторизацији тескта. Његове варијације, \textit{RoBERTa}\footnote{\textit{Robustly Optimized BERT} -- Робусно оптимизовани \textit{BERT}}~\citep{liu2019roberta} и \textit{DeBERTa}\footnote{\textit{Decoding-Enhanced BERT} -- Декодерски-побољшани \textit{BERT}}~\citep{he2020deberta} и данас постављају најбоље резултате на задацима угњежђавања речи (\textit{word embedding}), анотацијa речи (нпр. обележавање врсте речи и и препознавање именованих ентитета) и класификације реченица и докумената. Са друге стране, појављивање модела \textit{GPT} (генеративни предобучени трансформер)~\citep{radford2018improving} и \textit{GPT-2}~\citep{radford2019language} је популаризовало језичке моделе засноване на траснформерском декодеру, а ова групација модела је она која се данас најбрже развија. Модели који комбинују употребу енкодера и декодера, као што су, на пример \textit{BART}~\citep{lewis2020bart} и \textit{T5}~\citep{raffel2020exploring}, остају недовољно запажени упркос изванредним резултатима које постижу на задацима трансформације текста, као што су машинско превођење, сумaризација и прилагођавањe стила.

%%% Почетком двадесет и првог века, дошло је најпре до наглог пораста количине доступних текстуалних података, а потом и до наглог раста рачунарске моћи, што је узроковало талас истраживања заснованих на идеји дубоког учења (\textit{deep learning})~\citep{lecun2015deep}. У случају обраде природних језика, истраживања кулминирају појавом архитектуре трансформера~\citep{vaswani2017attention}, која се базира на употреби енкодера, чија је главна намена анализа тескта, и декодера, чија је главна намена синтеза тескта. Ипак, први опште популаран модел базиран на овој архитектури био је \textit{BERT}\footnote{\textit{Bidirectional Encoder Representations from Transformers} -- двосмерно кодирање репрезентације из трансформера}~\citep{devlin2018bert}, заснован искључиво на трансформерском енкодеру. Овај модел је направио велики помак у обради природног језика, пре свега на задацима који се заснивају на векторизацији тескта. Његове варијације, \textit{RoBERTa}\footnote{\textit{Robustly Optimized BERT} -- Робусно оптимизовани \textit{BERT}}~\citep{liu2019roberta} и \textit{DeBERTa}\footnote{\textit{Decoding-Enhanced BERT} -- Декодерски-побољшани \textit{BERT}}~\citep{he2020deberta} и данас постављају најбоље резултате на задацима угњежђавања речи (\textit{word embedding}), анотацијa речи (нпр. обележавање врсте речи и и препознавање именованих ентитета) и класификације реченица и докумената. Са друге стране, појављивање модела \textit{GPT} (генеративни предобучени трансформер)~\citep{radford2018improving} и \textit{GPT-2}~\citep{radford2019language} је популаризовало језичке моделе засноване на траснформерском декодеру, а ова групација модела је она која се данас најбрже развија. Модели који комбинују употребу енкодера и декодера, као што су, на пример \textit{BART}~\citep{lewis2020bart} и \textit{T5}~\citep{raffel2020exploring}, остају недовољно запажени упркос изванредним резултатима које постижу на задацима трансформације текста, као што су машинско превођење, сумaризација и прилагођавањe стила.

\subsection{Преглед објављених модела за српски језик}
Језички модели засновани на архитектури трансформера су направили продор у српски језик путем вишејезичних модела, најпре кроз \textit{MBERT}\footnote{\textit{Multilingual BERT} -- вишејезични \textit{BERT}}~\citep{devlin2018bert}, а потом и кроз \textit{XLM-RoBERTa}\footnote{\textit{Cross-lingual Language Model} -- Међујезички језички модел} модел~\citep{conneau2019unsupervised}, за чије обучавање је коришћено око 4 милијарде токена из тесктова писаних на српском или другом блиско-сродном језику (хрватски, босански). Потоњи модел објављен је у децембру 2019. године у две варијанте, \textit{base} (279 милиона параметара) и \textit{large} (561 милион параметара). И данас се, као један од највећих модела за векторизацију, употребљава у обради српског језика и притом остварује добре резултате, поготово након дообучавања.

Почетком 2021. године, на платформи \textit{Huggingface}\footnote{Највеће веб чвориште за објављивање језичких модела, \href{https://huggingface.co}{huggingface.co}} објављен је  модел под називом \textit{БЕРТић} (\textit{classla/bcms-bertic})~\citep{ljubevsic2021berti}, базиран на архитектури \textit{ELECTRA}~\citep{clark2020electra}, са 110 милиона параметара, обучаван на корпусу од преко 8 милијарди токена, босанског (800 милиона), хрватског (5.5 милијарди), црногорског (80 милиона) и српског језика (2 милијарде).

Касније те исте године, објављени су први модели направљени специфично за српски језик у оквиру једног ширег језичког истраживања за македонски језик~\citep{dobreva2022macedonizer}. Прецизније, објављена је српска верзија \textit{RoBERTa-base} модела, \textit{macedonizer/sr-roberta-base} (120 милиона параметара) и српска верзија \textit{GPT2-small} модела, \textit{macedonizer/sr-gpt2} (130 милиона параметара). Оба модела су обучавана на корпусу српске Википедије и подржавају само ћирилично писмо.

Недуго потом предузет је сличан подухват, при којем је обучено пет \textit{RoBERTa-base} модела за српски језик~\citep{cvejic2022prepoznavanje}. Иницијални модел, \textit{Andrija/SRoBERTa}, имао је 120 милиона параметара и обучаван је на малом корпусу од 18 милиона токена познатом под именом \textit{Leipzig}~\citep{biemann2007leipzig}, док су потоња четири модела имала по 80 милиона параметара и обучавана су инкрементално на све већем и већем корпусу. За модел \textit{Andrija/SRoBERTa-base} додат је корпус \textit{OSCAR}~\citep{suarez2019asynchronous} (220 милиона токена), за модел \textit{Andrija/SRoBERTa-L} је поред њега додат и \textit{srWAc}~\citep{ljubevsic2014bs} (490 милиона токена), а за моделе \textit{Andrija/SRoBERTa-XL} и \textit{Andrija/SRoBERTa-F} су уз претходне додати и корпуси \textit{cc100-hr} (21 милијарда токена) и \textit{cc100-sr} (5.5 милијарди токена)~\citep{wenzek-etal-2020-ccnet}, у мањој и већој мери.

Крајем 2022. године објављено је три експериментална генеративна модела за српски језик~\citep{vskoric2023композитне}. Контролни модел, \textit{procesaur/gpt2-srlat} заснован је, поново, на \textit{GPT2-small} архитектури, има 138 милиона параметара и обучен је на исечку корпуса Друштва за језичке ресурсе и технологије (260 милиона токена)~\citep{krstev2022deliverable}. Друга два модела, \textit{procesaur/gpt2-srlat-sem} и \textit{procesaur/gpt2-srlat-synt}, настала су дообучавањем првог коришћењем два специјално припремљена корпуса са циљем моделовања семантике или синтаксе текста засебно. Tри модела су потом употребљена за експеримент комбиновања језичких модела на задатку класификације реченица~\citep{vskoric2023transformer}.

Почетком наредне године, истраживачи са Универзитета у Нишу објављују модел \textit{JelenaTosic/SRBerta} (120 милиона параметара), заснован поново на  \textit{RoBERTa-base} архитектури и обучаван помоћу корпуса \textit{OSCAR}~\citep{suarez2019asynchronous}. Оно што је занимљиво за овај модел, али и за другу верзију објављену под именом \textit{nemanjaPetrovic/SRBerta} је да су пре објављивања они дообучени над текстовима из домена права~\citep{bogdanovicsrberta}. У периоду између објављивања ова два модела, објављен је и \textit{aleksahet/xlm-r-squad-sr-lat}~\citep{cvetanovic2023synthetic}, први модел за одговарање на питања на српском језику, настао прилагођавањем \textit{XLM-RoBERTа} модела помоћу скупа података \textit{SQuAD}~\citep{rajpurkar2018know} преведног на српски језик.

Средином 2023. године објављена су још два генеративна модела заснована на ГПТ архитектури. Оба модела су обучавана над истим скупом података: над корпусима Друштва за језичке ресурсе и технологије~\citep{krstev2022deliverable}, докторским дисертацијама преузетим са платформе НАРДУС\footnote{Национални Репозиторијум (докторских) Дисертација (са свих универзитета) у Србији, \href{https://nardus.mpn.gov.rs/}{nardus.mpn.gov.rs}}, корпусу јавног дискурса српског језика Института за српски језик САНУ под називом \textit{PDRS}~\citep{11356/1752} и додатним јавно доступним, али филтрираним веб корпусима као што су већ поменути \textit{srWAc}~\citep{ljubevsic2014bs} и \textit{cc100-sr}~\citep{wenzek-etal-2020-ccnet}. Укупан број токена у овом скупу података броји око 4 милијарде токена. Већи модел, \textit{jerteh/gpt2-orao}\footnote{\href{https://huggingface.co/jerteh/gpt2-orao}{huggingface.co/jerteh/gpt2-orao}}, броји 800 милиона параметара, заснован је на архитектури \textit{GPT2-large} и представља тренутно највећи достпуни модел предобучен за српски језик. Мањи модел, \textit{jerteh/gpt2-vrabac}\footnote{\href{https://huggingface.co/jerteh/gpt2-vrabac}{huggingface.co/jerteh/gpt2-vrabac}}, броји 136 милиона параметара и заснован је на архитектури \textit{GPT2-small}. Оба модела су обучавана коришћењем рачунарских ресурса Националне платфроме за вештачку интелигенцију Србије. Осим корпуса за обучавање, ова два модела деле и речник токена и токенизатор, специјално опремљен да изједначава ћирилично и латинично писмо, омогућујући њихову равноправну подршку.

Након објављивања генеративног модела од 800 милиона параметара фокус истраживачких група се полако помера на дообучавање великих модела коришћењем текстова на српском језику. Па су тако објављена два модела заснована на архитектури \textit{Alpaca}~\citep{taori2023alpaca}, \textit{datatab/alpaca-serbian-3b-base} (3 милијарде параметара) и \textit{datatab/alpaca-serbian-7b-base} (7 милијарди параметара), a најављено је и објављивање још једног модела исте величине, заснованог на архитектури \textit{Mistral-7b}~\citep{jiang2023mistral}, који је обучаван на хрватским, босанским и српским текстовима који броје 11.5 милијарди токена.
Исти корпус од 11.5 милијарди токена коришћен је и за дообучавање \textit{XLM-RoBERTa-large} модела у циљу поређења перформанси дообучаваних модела у односу на моделе који су обучавани \textit{од нуле}. Нови модел је објављен под именом \textit{classla/xlm-r-bertic} и броји 561 милион параметара, колико има и оригинални \textit{XLM} модел.

Коначно, на скупу података над којим су обучавани \textit{jerteh/gpt2-orao} и \textit{jerteh/gpt2-vrabac}, обучена су још два модела за векторизацију текста. Већи модел, \textit{jerteh/Jerteh-355}\footnote{\href{https://huggingface.co/jerteh/jerteh-355}{huggingface.co/jerteh/jerteh-355}}, заснован је на \textit{RoBERTa-large} архитектури и броји 355 милиона параметара, док је мањи модел, \textit{jerteh/Jerteh-125}\footnote{\href{https://huggingface.co/jerteh/jerteh-125}{huggingface.co/jerteh/jerteh-125}}, заснован је на \textit{RoBERTa-base} архитектури и броји 125 милиона параметара. Као и код модела \textit{jerteh/gpt2-orao}, циљ је био да се модели обуче на што квалитетнијем корпусу текстова. У наставку рада, перформансе ова два модела ће бити испитане и поређене са перформансама других, одабраних модела, како би се установила њихова места у хијерахији језичких модела за векторизацију текста на српском језику.


\subsection{Поставка експеримента}
У претходном одељку установљено је да постоји већи број вишејезичних модела са подршком за обраду српског језика, у мањој или већој мери, али и да постоји двадесетак модела који су припремљени специјално за ту намену. Објављени модели се међусобно разликују према неколико особина: породици (архитектури) модела и броју његових параметара, речнику/токенизатору на којем се заснивају, скупу који је коришћен за њихово обучавање, задатку на којем је модел обучаван и дужини обучавања. Треба напоменути и да неке од ових информација недостају за неке од модела, али и да су неке информације које су доступне (пре свега особине скупа који је коришћен за обучавање) непроверљиве.

У наставку рада фокус ће бити на десет одабраних модела за векторизацију (општег типа). Биће представљене основне информације о тим моделима (Одељак~\ref{sec:2}), и биће приказан експеримент поређења њихових перформанси на четири припремљена задатка (Одељак~\ref{sec:3}). Резултати четири експеримента ће бити приказани и размотрени (Одељак~\ref{sec:4}) и, напослетку (Одељак~\ref{sec:5}), биће дат предлог за процес обучавања нових модела за српски језик. Овај рад се неће фокусирати на генеративне моделе услед недостатка поузданог (али аутоматског) механизма за мерење њихових перформанси. Још увек није објављен ниједан енкодер-декодер модел специјално за српски језик.


==> settings/right/settings.tex <==
% ----------- update from the preamble % -------------

% jezici
\usepackage[english]{babel}
% kodne strane
\usepackage[T1,T2A]{fontenc} 
\usepackage[utf8]{inputenc} 

%\usepackage{indentfirst}
%\usepackage{lmodern}

\usepackage{csquotes}

\usepackage{amsmath}
\usepackage[authordate,backend=biber,dashed=false]{biblatex-chicago}


%
% ------------ biblioteke ----------

% specificne dimenzije stranica
\usepackage{geometry}
 \geometry{
	top=23mm,
	bottom=21mm,
	left=12mm,
	right=20mm
 }
% slike
\usepackage{graphicx}
% putanja do direktorijuma sa slikama
\graphicspath{ {images/color/} }
% proizvoljne boje
\usepackage[dvipsnames]{xcolor}
% poravnanje teksta
\usepackage{ragged2e}
% dupla linija u tabeli
\usepackage{array}
% zbog adjustwidth svojstva
\usepackage{changepage}
% podesavanje zaglavlja
\usepackage{fancyhdr}
% definicija okruzenja koje koristi parbox-ove
%% ne moze klasican nacin jer ne dozvoljava nebalansirane zagrade
\usepackage{environ}
% linkovi
\usepackage[colorlinks = true,
            linkcolor = Sepia,
            urlcolor  = Mahogany,
            citecolor = BrickRed,
            anchorcolor = Sepia]{hyperref}
% fusnote
\usepackage{footnote}
\makesavenoteenv{tabular} %% fusnote "znaju" da ne rade u tabelama

%
% ------------ podesavanje fonta ----------
%
%\renewcommand\familydefault{\sfdefault} %% deluje neozbiljno

% debljina linije zaglavlja
\renewcommand{\headrulewidth}{0.4pt}

%
% ----------------- boje -------------------------
%
\definecolor{light_gray}{rgb}{0.5, 0.5, 0.5}
\definecolor{dark_gray}{rgb}{0.4, 0.4, 0.4}
\definecolor{darker_gray}{rgb}{0.2, 0.2, 0.2}

%
% ----------------- definicije novih naredbi ---------------
%
% 

%%%%% UDK %%%%%%%%
\newcommand{\udk}[1]{\begin{adjustwidth}{-0.5cm}{}{\par\textcolor{dark_gray}{\parbox{\textwidth}{\begin{flushright}\texttt{УДК #1}\end{flushright}}}}\end{adjustwidth}}

% autor
\renewcommand{\author}[1]{\hfill #1 \newline}
% institution
\newcommand{\institution}[1]{
	\textcolor{darker_gray}{\textit{\small \hfill #1}} \newline
}
% email
\renewcommand{\email}[1]{\textcolor{light_gray}{\hfill \small #1} \newline}

% prevod s engleskog
\newcommand{\srtranslation}[2]{%
		\vspace{#1cm}
		\parbox[t]{0.4\textwidth}{
			\hfill \textit{\textcolor{darker_gray}{Превод с енглеског:}} 
				\begin{flushright}#2\end{flushright}
		}	
}%

%
% ----------------- redefinicije postojecih naredbi ---------------
%
% naslov
\renewcommand{\title}[1]{\begin{center}\Large\bfseries\boldmath#1\end{center}}


%
% ----------------- definicija novih okruzenja ---------------
%
% okruzenje za glavni deo = apstrakt, datumi, autori, prevod (sve)
\newenvironment{main}
		{\begin{adjustwidth}{-0.2cm}{}\begin{tabular}{ l @{~} @{~} !{\vrule width 2pt}| @{~} l }}
		{\end{tabular}\end{adjustwidth}}
% okruzenje za apstrakt
\NewEnviron{abstractenv}{%
	 %\vspace{-1cm}  %% fix zbog margina apstrakta
		%  sazetak  
		\parbox[t]{0.6\textwidth}{	
			\begin{adjustwidth}{-1cm}{}	
				\begin{abstract}							
					% tekst sazetka
					\BODY						
				\end{abstract}
			\end{adjustwidth}
		}
}% 
% podaci o autorima
\NewEnviron{authorsenv}{%
  \parbox[t]{0.4\textwidth}{%
      \BODY
   }
}%  
